Certified Adversarial Defenses Meet Out-of-Distribution Corruptions: Benchmarking Robustness and Simple Baselines

Certified robustness guarantee gauges a model's robustness to test-time attacks and can assess the model's readiness for deployment in the real world. In this work, we critically examine how the adversarial robustness guarantees from randomized smoothing-based certification methods change when state-of-the-art certifiably robust models encounter out-of-distribution (OOD) data. Our analysis demonstrates a previously unknown vulnerability of these models to low-frequency OOD data such as weather-related corruptions, rendering these models unfit for deployment in the wild. To alleviate this issue, we propose a novel data augmentation scheme, FourierMix, that produces augmentations to improve the spectral coverage of the training data. Furthermore, we propose a new regularizer that encourages consistent predictions on noise perturbations of the augmented data to improve the quality of the smoothed models. We find that FourierMix augmentations help eliminate the spectral bias of certifiably robust models enabling them to achieve significantly better robustness guarantees on a range of OOD benchmarks. Our evaluation also uncovers the inability of current OOD benchmarks at highlighting the spectral biases of the models. To this end, we propose a comprehensive benchmarking suite that contains corruptions from different regions in the spectral domain. Evaluation of models trained with popular augmentation methods on the proposed suite highlights their spectral biases and establishes the superiority of FourierMix trained models at achieving better-certified robustness guarantees under OOD shifts over the entire frequency spectrum.

==> sections/3-preliminary.tex <==
\section{Preliminaries}
\label{sec:prelim}

\noindent \textbf{Problem Statement.}\quad The standard image classification task involves an underlying data distribution $\mathcal{D}$ with samples $\vx \in \mathcal{X} \subset \sR^{d\times d}$ and their corresponding labels $y \in \mathcal{Y} \subset \sR^{+}$.
Usually $\mathcal{D}$ is unknown and the only accessible data is a training subset $\mathcal{D}_{train}$ that is an \textit{i.i.d} sample from $\mathcal{D}$. 
The trained classifier $\mathcal{M}$ is expected to perform well on $\mathcal{D}$.
However, real-world test images oftentimes do not follow the same/clean distribution $\mathcal{D}$. 
Thus, the performance of $\mathcal{M}$ on out-of-distribution (OOD) data $\{(\hat{\vx},y)_1,...,(\hat{\vx},y)_n\} \sim \hat{\mathcal{D}}$ becomes a major consideration. 
Another key aspect of robustness is performance of the model $\mathcal{M}$on adversarial examples. 
$\vx' = \vx + \vdelta$ is an adversarial example if the model $\mathcal{M}$ incorrectly predicts the class of $\vx'$. 
Following previous works~\cite{cohen2019certified}, we target the $\ell_2$ robustness in that we call the model $\mathcal{M}$ to be ${robust}_{\ell_2}(\vx,y,\epsilon)$  at radius $\epsilon$ if it predicts $\vx$ correctly for any $\vx+\vdelta$ such that $||\vdelta||_2<\epsilon$. 
In this work, we take the first steps to benchmark and improve the certified robustness of $\mathcal{M}$ on OOD data, \ie ${robust}_{\ell_2}(\hat{\vx},y,\epsilon)$.

\noindent\textbf{Certified Radius.}\quad Previous works have proposed theoretical guarantees of the model's robustness by deriving tight lower bounds on $\epsilon$ that achieves ${robust}_{\ell_2}(\vx,y,\epsilon)$ for a model $\mathcal{M}$. 
Such a lower bound is defined and denoted as \textit{certified radius}~\cite{Zhai2020MACER} ($\text{CR}(\mathcal{M},\vx;y)$). 

\noindent\textbf{Randomized Smoothing.}\quad Our work focuses on the most scalable certifiable defense framework, randomized smoothing (RS)~\cite{cohen2019certified}.
The core of RS is to transform classifier $\mathcal{M}$ to its smoothed version $\hat{\mathcal{M}}$ by: 
\begin{equation}
    \hat{\mathcal{M}}(\vx) = \argmax_{c \in \mathcal{Y}}\sP(\mathcal{M}(\vx+\vdelta)=c), \vdelta \sim \mathcal{N}(0,\sigma^{2}\mathbf{I}).
    \label{eq:rs}
\end{equation}
$\hat{\mathcal{M}}$ returns the most probable class returned by $\mathcal{M}$ on Gaussian perturbations ($\mathcal{N}(0,\sigma^{2}\mathbf{I})$) of the input $\vx$.
Cohen \etal~\cite{cohen2019certified} showed that predictions of $\hat{\mathcal{M}}$ are consistent in the $\ell_2$ radius of:  
\begin{equation}
   \text{CR}(\hat{\mathcal{M}},\sigma,\vx;y) = \frac{\sigma}{2}(\Phi^{-1}(p_A)-\Phi^{-1}(p_B)),
   \label{eq:cr}
\end{equation}
where $\Phi^{-1}$ is the inverse of standard Gaussian CDF and we denote $c_A$ as the returned prediction of the base classifier $\mathcal{M}$ with probability $p_A=\sP(\mathcal{M}(\vx+\vdelta)=c_{A})$ and $c_B$ is the runner-up prediction with probability $p_B=\max_{c \neq c_{A}} \sP(\mathcal{M}(\vx+\vdelta)=c_{A})$. Monte Carlo-based sampling~\cite{hammersley2013monte} is utilized to approximate $\underline{p_A} \leq p_A$ and $\overline{p_B} = 1-\underline{p_A} \geq p_B$. The proof of Equation~\ref{eq:cr} still holds if we replace $p_A$ and $p_B$ with $\underline{p_A}$ and $\overline{p_B}$, respectively.    

\noindent\textbf{Fourier Analysis.}\quad 2D images can be converted into the frequency domain by Fourier transform $\mathcal{F}(\cdot)$ and vice versa. Fourier transform has the \textit{duality} property, which provides a unique but equivalent perspective for image analysis. We leverage fast Fourier transform (FFT) and inverse FFT (IFFT) in our study for the transformation between the pixel and frequency domains. $\text{FFT}(\vx)$ is complex in general, \ie $\text{FFT}(\vx)= \text{FFT}_{real}(\vx)+i\text{FFT}_{imag}(\vx)$, with $\mA = |\text{FFT}(\vx)|$ is its amplitude spectrum and $\mP = \arctan(\text{FFT}_{imag}(\vx)/\text{FFT}_{real}(\vx))$ is its phase spectrum.


\noindent\textbf{Benchmark Datasets.}\quad We utilize CIFAR-10/100~\cite{krizhevsky2009learning} datasets consisting of small $32 \times 32 \times 3$ natural images, both with 50,000 training and 10,000 testing images in our study.  We also use ImageNet~\cite{deng2009imagenet} that consists of 1.2 millions images with 1,000 classes. We crop images in ImageNet into the same size of $224\times224\times3$ pixels. Since we focus on the certified robustness under OOD shifts, we use CIFAR-10/100-C, CIFAR-10/100-$\overline{\text{C}}$, ImageNet-C, and ImageNet-$\overline{\text{C}}$ for our OOD performance evaluation~\cite{hendrycks2019benchmarking,mintun2021interaction}.


\noindent\textbf{Metrics.}\quad We use \textit{average certified radius} (ACR) to evaluate the certified robustness of RS, namely $\text{ACR}:=\frac{1}{|\mathcal{D}_{test}|}\sum_{(\vx,y)\in \mathcal{D}_{test}} \text{CR}(\hat{\mathcal{M}},\sigma,\vx;y)\times\textbf{1}_{\hat{\mathcal{M}}(\vx,\sigma)=y}$. It is worth noting that we assign $\text{CR}(\cdot)=0$ for incorrect prediction of $\hat{\mathcal{M}}$. ACR is thus a comprehensive metric to measure the certified robustness and utilized in most prior arts as well~\cite{Zhai2020MACER,salman2019provably}. We also measure the mean corruption ACR (mACR) as an overall metric, $\text{mACR} := \frac{1}{c}\sum_{i=1}^{c}{\text{ACR}_{i}}$, where $c$ is the number of corruptions leveraged in a specific test set. For example, $c=15$ and $10$ in CIFAR-10/100-C and -$\overline{\text{C}}$ datasets, respectively. Unlike previous studies we do not use the \textit{empirical} clean and robust accuracy~\cite{cohen2019certified,salman2019provably,Zhai2020MACER} as a metric in this work since we focus on the \textit{certified} robustness. In~\S~\ref{sec:rs_on_c}, we demonstrate that empirical and certified robustness on OOD data are not correlated with each other.

% {\color{red}{Define CR=0 for wrong prediction and we do not report ACA at r=0. Justify why we are no longer interested in empirical clean and corrupted accuracies. Or why empirical robust advances do not translate to certified robustness. Cite Table 2, Figure 9 and Figure 12 of AugMix for consistent gain on all corruption types or plots from Akshay.
% CR SOTAs are surprisingly vulnerable compared to ER SOTAs from RobustBench -- keep in mind that Fig 1 models were designed for in-dist robustness unlike robustbench model so use this argument carefully. The issue is with CR methods and not fundamental to the hardness of perturbations.
% }}

==> sections/4-analysis.tex <==
\section{RS-Based Certified Defenses Under Common Corruptions}
To apply randomized smoothing (RS) technique, the base classifier $\mathcal{M}$ is desired to be robust against Gaussian noise (see Eq.~\ref{eq:rs}), though the result of Eq.~\ref{eq:cr} holds regardless how $\mathcal{M}$ is trained. The robustness and correctness of the smoothed classifier $\hat{\mathcal{M}}$ relies on the consistent prediction of $\mathcal{M}$ on $\mathcal{N}(\vx,\sigma^2 \mathbf{I})$ as $\vx$'s correct label $y$.
Intuitively, Cohen~\etal propose to leverage Gaussian augmentation to train the base classifier at variance $\sigma^2$~\cite{cohen2019certified}. SmoothAdv~\cite{salman2019provably} and MACER~\cite{Zhai2020MACER} both use Gaussian augmentation and further improve Cohen~\etal's baseline method by adversarial training and introducing an auxiliary objective to maximize the certified radius, respectively. However, the certification performances of these certifiable defenses on OOD data are left unexplored. 
We thus take the first step to evaluating Gaussian, SmoothAdv, and MACER on CIFAR-10-C and further compare their provided certified robustness on CIFAR-10. As Table~\ref{tb:1} shows, SmoothAdv and MACER both achieve tangible enhancements of ACR on CIFAR-10 compared to the Gaussian augmentation baseline, but fail to deliver satisfactory certified robustness on CIFAR-10-C. The drops are more than 20\% for all three methods. SmoothAdv and MACER suffer similar relative drops between the certification performance on CIFAR-10 and CIFAR-10-C with the baseline method. 

\begin{table}[h]
\scriptsize
\renewcommand\arraystretch{1.}
\setlength\tabcolsep{4.8pt}
\vspace{-0.25cm}
  \caption{\small ACR and mACR of CIFAR-10-C with $\sigma=0.25$. }
  \label{tb:1}
  \vspace{-0.25cm}
  \centering
  \begin{tabular}{|l|c|c|c|}
\noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}

    Method    &CIFAR-10 $\uparrow$ (ACR) &CIFAR-10-C $\uparrow$ (mACR) & Drop $\downarrow$ (\%)\\
\noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
    Gaussian    &0.461 &0.363 & 21.3\\
    SmoothAdv    &0.519 &0.411 &\textbf{20.8} \\
    MACER    &\textbf{0.539} &\textbf{0.426} & 21.0 \\
\noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}

  \end{tabular}
  \vspace{-0.25cm}
\end{table}

The results in Table~\ref{tb:1} indicate that there are serious problems in SOTA RS-based methods on certifying OOD data, though they have achieved high ACR on in-distributional data. Unfortunately, the real-world data is not oftentimes from the same distribution with the training set, rendering SOTA methods less effective. It is, therefore, important to study the underlying reason of the failure and how to improve the certification on OOD data.
% Test-time adaptation based methods are generally not since they requires the models dynamic change. However Theorem 1 a deterministic base classifier. We demonstrate their ineffectiveness in \S~\ref{}.

% {\color{red}{Empirical accuracy and computational complexity: Compared to FourierMix, macer and smoothadv does very poorly on both of these metrics however similar in ACR. Think of motivation for these metrics in RS based defenses as well.}}



% \begin{figure*}[t]
% \begin{center}
% \includegraphics[width=\linewidth]{images/fig1.png} 
% \end{center}
% \caption{Average Certified Radius (ACR).\BK{Should we mention average drop in performance and noise, blur, weather, and digital category instead? New grouping looking at the PSDs.} Jiachen: try different things and see the figures.}
% \end{figure*}

% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=\linewidth]{images/fig2.png} 
% \end{center}
% \caption{Motivation: Empirical Robust Accuracy. Dan: show full results in the appendix. Use simplified in main paper. Possibly just look at severity five comparisons so that we do not need to process so many bars. Possibly just compare high and low. Maybe just compare one method/the best method. We want to convey that ACR methods are fragile.}
% \end{figure}

\subsection{Analyzing the Brittleness of Smoothed Classifiers Through a Spectral Lens}

\BK{In this section, we ask the question: what is a common feature among the Group 3 corruption types? Answering this question may help us identify the drawbacks of existing certifiable defense schemes and design appropriate countermeasures.}


As mentioned above, since the base classifier $\mathcal{M}$ needs to be robust against Gaussian noise for RS, Gaussian augmentation becomes a gold standard for all RS-based methods, which have helped achieve good certified robustness on in-distributional data. On the other hand, Yin~\etal recently study the empirical robustness of DNNs from the Fourier perspective and show that Gaussian augmented models are biased to be robust against high frequency perturbations~\cite{yin2019fourier}. This motivates us to rethink the RS-based certification methods from the Fourier perspective. Specifically, we empirically group the 15 corruptions in CIFAR-10-C to three categories (\ie low, mid, and high frequency corruptions) based their $\mathbb{E}[|\text{FFT}(C(\vx)-\vx)|]$, where $C(\cdot)$ is the corruption function. The low frequency corruptions have \{\texttt{brightness}, \texttt{fog}, \texttt{frost}, \texttt{snow}, \texttt{contrast}\}; mid frequency corruptions have \{\texttt{defocus blur}, \texttt{frosted glass blur}, \texttt{motion blur}, \texttt{zoom blur}, \texttt{elastic}\}; and  high frequency corruptions have \{\texttt{Gaussian noise}, \texttt{impulse noise}, \texttt{shot noise}, \texttt{pixelate}, \texttt{JPEG}\}. We visualize their $\mathbb{E}[|\text{FFT}(C(\vx)-\vx)|]$ in Appendix~\ref{}.

Figure~\ref{fig:motivation1} shows the mACR of three RS-based methods on three categories with different severity levels in CIFAR-10-C. It is clear that RS-based certification is extremely vulnerable to \textbf{low-to-mid} frequency corruptions, where the mACRs drastically degrade xx-xx\%. To confirm that the degradation comes from the certification methodologies, we select three SOTA empirical defense methods~\cite{hendrycks2019augmix,kireev2021effectiveness,rebuffi2021fixing} and evaluate them on the same categories in CIFAR-10-C. Figure~\ref{fig:motivation2} shows the results. We find the empirical robust accuracy remains reasonably high even with high severity levels. 

The observations can be explained by the high frequency bias in the base classifier $\mathcal{M}$. If $C(\vx)-\vx$ lies in high frequencies, so will $C(\vx)-\vx+\vdelta$, and $\hat{\mathcal{M}}$ is expected to perform well on those corruption types. However, the low-to-mid frequency corruptions will shift the overall perturbation $C(\vx)-\vx+\vdelta$ to much lower frequencies. Gaussian augmented models thus have high error rates~\cite{yin2019fourier} on those corruptions.

\begin{figure}[h]
\vspace{-0.3cm}
% \captionsetup[sub]{font=tiny,labelfont={bf,sf}}
\subfigure[Gaussian \label{fig:}]{\begin{minipage}[t]{0.325\linewidth}
\begin{center}
\includegraphics[width=\linewidth]{images/incorrect_radius_hm_ga.png} 
\end{center}
\end{minipage}}
\subfigure[SmoothAdv \label{fig:}]{\begin{minipage}[t]{0.325\linewidth}
\begin{center}
\includegraphics[width=\linewidth]{images/smoothadv_heatmap.png} 
\end{center}
\end{minipage}}
\subfigure[MACER \label{fig:}]{\begin{minipage}[t]{0.325\linewidth}
\begin{center}
\includegraphics[width=\linewidth]{images/macer_heatmap.png} 
\end{center}
\end{minipage}}
\vspace{-0.4cm}
\caption{Reasoning of Failure: Average Certified Radius (ACR) of Fourier Basis Analysis on CIFAR-10 with $\epsilon = 4$.}
\label{fig:fourier_basis1}
\vspace{-0.25cm}
\end{figure}


Furthermore, we leverage the Fourier basis analysis~\cite{yin2019fourier} to cross-validate our reasoning. We first briefly introduce the Fourier basis analysis method. A Fourier basis in the pixel space is a real-valued matrix $\mU_{i,j} \in \sR^{d\times d}$ where its $||\mU_{i,j}||_2 = 1$ and $\text{FFT}(\mU_{i,j})$ only has two non-zero elements at $(i,j)$ and $(-i,-j)$ in the coordinate that views the image center as the origin. Given a test set and a smoothed model, we evaluate the ACR of the model on $\widetilde{\vx_{i,j}} = \vx + r\epsilon \mU_{i,j}$ for each $\vx$ in the test set, where $r$ is randomly sampled in $\{-1,1\}$ and $\epsilon$ is the $\ell_2$ norm. Each of the evaluated ACR will correspond to a data point in the heat map located $(i,j)$. It is worth noting each data point (\ie ACR) is evaluated on the perturbed test set but not on a single perturbed image. Figure~\ref{fig:fourier_basis1} shows the heat maps of Gaussian, SmoothAdv, and MACER using $\epsilon=4$. Informally, the center and edges of the heat map contain evaluation on the lowest and highest frequency perturbations, respectively.  Such results confirm the vulnerability of low-to-mid frequency corruptions. The ACRs are always less than 0.3 for all three methods in the low-to-mid frequency range, while they perform well in high frequency areas.

% Motivate the use of FourierMix. We dont need domain input making it more general and less prone to overfitting to overfitting to base corruption types. Gaussian augmentation overfits to high frequency corruptions and AugMix overfits to low frequency corruptions. FourierMix improves performance on all frequencies. From perceptual similarity to spectral diversity -- how to show that these issues are arising because augmentations are spectrally biased and motivate the need for spectrally diverse augmentations. 

%{\color{red}{Heatmap of Gaussian, MACER, smothAdv highlighting susceptibility in low frequency regime.}}

==> sections/TODO.tex <==
\section{TODO:}
\begin{itemize}
    % \item Finish ImageNet-c and ImageNet-bar experiments (by supp mat deadline).
    \item Our Discussion/Explanation should be contrasted with the Fourier perspective paper as scientific applications may have more mid-high frequency noise.
    % \item Justify how results of evaluating on CIFAR10-F are better than those of evaluating on CIFAR10-C in terms of OOD robustness. 
    % (Can we say something like evaluating on CIFAR10-F helps to give a fair comparison of evaluation on true OOD data?)
    % \item Perform ranking experiments using RobustBench models on both cifar-10/100-bar and cifar-10-f.
    % \item Teaser image and image for Fourier-Mix + HCR.
    % \item Add full gaussian JSD and HCR comparison for FourierMix in Supp Mat.
    % \item If time permits, plot heatmap for one deterministic l2 certification in Supp Mat.
    % \item Add clean numbers in all tables for all method
    \item Work on Dan's suggestions
    \item ImageNet-R experiments
    \item Rebuttal: AugMix + HCR and Augmix + FourierMix
    \item Cifar-10/100-f average tables. 
    
    \item some citations: https://arxiv.org/pdf/2006.16241.pdf,
    icml 2020 paper
    
    \item ablations on the fouriermix
\end{itemize}

\if0
1. Finish ImageNet experiments
2. Discussion on the Fourier perspective paper.
3. argue that cifar10-f is natural/common in terms of formulation
scientific applications may have more mid-high frequency noise.
ImageNet-R
foureirmix's distribution
batch-wise
Dan Hendrycks1:40 PM
ImageNet-R
Dan Hendrycks1:59 PM
x * unif
x + normal
x {+, *} {unif, tent, normal, * (1 + normal)}

robustmix comparison

HCR 

cifar10-f can be auxiliary 
\fi



==> sections/backuptables.tex <==
\begin{table*}[t]
\scriptsize
\renewcommand\arraystretch{0.9}
\setlength\tabcolsep{2.5pt}
  \caption{\small Models trained with \emph{FourierMix} and HCR achieve significant improvements in the certified robustness (ACR) guarantees on all corruption types from the CIFAR-10-C dataset.  %$\sigma=0.25$ is used for certification with RS and model training.
  %for Different Data Augmentations. 
  \textbf{Bold} and \underline{underline} denote the best and runner-up results, for all tables in this work. 
  %\BK{Better caption with message/results -- eg see winning hand captions}\AM{Move the detailed result to Appendix and only keep first 5 columns.}
  }
  \label{tb:cifar10c}
  \vspace{-0.2cm}
  \centering
  \begin{tabular}{|l|c|cccc|}
    \noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}

    %Pretext Task     & Parameters  &Clean Accuracy &Adv. Accuracy  &Clean Accuracy &Adv. Accuracy  &Clean Accuracy &Adv. Accuracy\\
    Augmentation    &clean & mACR &-low &-mid &-high  \\
\noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}     
    Gaussian &0.461 & 0.363 &0.301 &0.353 &0.435 \\
     ~+JSD &\textbf{0.535} & 0.439 &0.346 &0.451 &\underline{0.520} \\
    \hline
     ~+AutoAugment &0.411  & 0.372 &0.312 &0.364 &0.431 \\
      ~~+JSD  &0.432 & 0.400 &0.343 &0.395 &0.464 \\
    \hline
     ~+AugMix &0.452 & 0.385 &0.324 &0.383 &0.449 \\
      ~~+JSD &0.518 & 0.430 &0.357 &0.436 &0.496 \\
      ~~+\textbf{HCR} &0.520 &0.437 &0.369 &0.444 &0.497\\
    \hline
     ~+\textbf{\emph{FourierMix}} &0.455 & 0.388 &0.326 &0.386 &0.453\\
      ~~+JSD &\underline{0.522} & \underline{0.444} &\underline{0.375} &\underline{0.454} &0.504\\
      
      ~~+\textbf{HCR} &\textbf{0.535} & \textbf{0.460} &\textbf{0.384} &\textbf{0.473} &\textbf{0.521}\\
\noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
  \end{tabular}
  \vspace{-0.2cm}
\end{table*}





\begin{table*}[h]
\scriptsize
\renewcommand\arraystretch{0.9}
\setlength\tabcolsep{2.0pt}
  \caption{\small Improvement in the Average Certified Radius (ACR) of models trained with \emph{FourierMix} and HCR against CIFAR-100-C corruptions.}
   \label{tb:cifar100c}
   \vspace{-0.2cm}
  \centering
  \begin{tabular}{|l|c|cccc|}
    \noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
    %Pretext Task     & Parameters  &Clean Accuracy &Adv. Accuracy  &Clean Accuracy &Adv. Accuracy  &Clean Accuracy &Adv. Accuracy\\
    Augmentation  & clean   & mACR &-low &-mid &-high  \\
    \noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
    Gaussian & 0.238 & 0.169 &0.131 &0.182 &0.208 \\
    ~+JSD & 0.291 & 0.232 &0.167 &0.248 &0.280 \\
    \hline
     ~+AutoAugment + JSD &0.265 & 0.225 &0.175 &0.234 &0.265\\
    \hline
     ~+AugMix + JSD & 0.286 & 0.231 &0.184 &0.240 &0.269 \\
     ~+AugMix + \textbf{HCR} &\underline{0.296}  &\underline{0.249} &\underline{0.191} &\underline{0.263} &\underline{0.292} \\
    \hline
     ~+\emph{FourierMix} + JSD &0.295 & 0.247 &0.190 &0.258 &\underline{0.292} \\
     ~+\textbf{\emph{FourierMix} + HCR} &\textbf{0.309} & \textbf{0.261} &\textbf{0.199} &\textbf{0.278} &\textbf{0.307} \\
\noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
  \end{tabular}
\end{table*}



\begin{table*}[h]
\scriptsize
\renewcommand\arraystretch{0.9}
\setlength\tabcolsep{2.25pt}
  \caption{\small Spectrally diverse augmentations from \emph{FourierMix} brings significant gains to certified robustness of the models trained on ImageNet against corruptions from ImageNet-C.
  %Average Certified Radius (ACR) of ImageNet-C with $\sigma=0.5$ Using Data Augmentations. 
  \AM{Keep first 5 columns and rest in Appendix}}
  \label{tb:imagenet-c}
  \vspace{-0.2cm}
  \centering
  \begin{tabular}{|l|c|cccc|}
\noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
    Augmentation  &clean & mACR &-low &-mid &-high  \\
\noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
    Gaussian &0.600 & 0.256 &0.155 &0.228 &0.385\\
    ~+JSD & 0.736 & 0.395 &0.220 &0.382 &\textbf{0.581} \\
    \hline
     ~+AugMix + JSD & 0.717 & 0.391 &0.238 &\underline{0.387} &0.550 \\
     ~+AugMix + \textbf{HCR} &0.727 &0.390 &0.234 &0.383 &0.552 \\
    \hline
     ~+\textbf{\emph{FourierMix}} + JSD &\textbf{0.751} &\textbf{0.399} &\textbf{0.242} &\textbf{0.389} &0.564 &0.515 \\
     ~+\textbf{\emph{FourierMix} + HCR} & \underline{0.750} &\underline{0.397} &\underline{0.239} &\underline{0.387} &\underline{0.567}\\
\noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
  \end{tabular}
\end{table*}


\begin{table*}[h]
\small
\renewcommand\arraystretch{0.9}
\setlength\tabcolsep{3pt}
  \caption{\small C-bar Results}
  \label{tb:cifar100c-bar}
  \vspace{-0.2cm}
  \centering
  \begin{tabular}{|l|c|c|c|c|}
\noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
    Augmentation     & CIFAR-10-$\bar{\text{C}}$  &CIFAR-100-$\bar{\text{C}}$  &ImageNet-$\bar{\text{C}}$  \\
\noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
    Gaussian & 0.314 &0.130 &0.266\\
    ~+JSD & 0.393 &0.196 &0.395\\
    \hline
     ~+AutoAugment + JSD & 0.346 & 0.176 & -\\
    \hline
     ~+AugMix + JSD & 0.382 & 0.193 &0.379\\
     ~+AugMix + \textbf{HCR} & 0.393 & \underline{0.211} &0.378\\
    \hline
    ~+\textbf{\emph{FourierMix}} + JSD & \underline{0.397} & 0.207 &\textbf{0.413}\\
     ~+\textbf{\emph{FourierMix} + HCR} &\textbf{0.419} & \textbf{0.227} &\underline{0.411}\\
\noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
  \end{tabular}
\end{table*}






  \centering
  \begin{tabular}{|l||c|cccc||c|cccc||c|cccc|}
    \noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
    & &\multicolumn{4}{c|}{CIFAR-10-C} & \multicolumn{4}{c|}{CIFAR-100-C} & \multicolumn{4}{c}{ImageNet-C} \\
    %Pretext Task     & Parameters  &Clean Accuracy &Adv. Accuracy  &Clean Accuracy &Adv. Accuracy  &Clean Accuracy &Adv. Accuracy\\
    Augmentation    &clean & mACR &-low &-mid &-high &clean & mACR &-low &-mid &-high &clean & mACR &-low &-mid &-high \\
\noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}     
    Gaussian &0.461 & 0.363 &0.301 &0.353 &0.435 & 0.238 & 0.169 &0.131 &0.182 &0.208 &0.600 & 0.256 &0.155 &0.228 &0.385\\
     ~+JSD &\textbf{0.535} & 0.439 &0.346 &0.451 &\underline{0.520}  & 0.291 & 0.232 &0.167 &0.248 &0.280 & 0.736 & 0.395 &0.220 &0.382 &\textbf{0.581}\\
    \hline
     ~+AutoAugment &0.411  & 0.372 &0.312 &0.364 &0.431 \\
      ~~+JSD  &0.432 & 0.400 &0.343 &0.395 &0.464 &0.265 & 0.225 &0.175 &0.234 &0.265 \\
    \hline
     ~+AugMix &0.452 & 0.385 &0.324 &0.383 &0.449 \\
      ~~+JSD &0.518 & 0.430 &0.357 &0.436 &0.496 & 0.286 & 0.231 &0.184 &0.240 &0.269 & 0.717 & 0.391 &0.238 &\underline{0.387} &0.550 \\
      ~~+\textbf{HCR} &0.520 &0.437 &0.369 &0.444 &0.497 &\underline{0.296}  &\underline{0.249} &\underline{0.191} &\underline{0.263} &\underline{0.292} &0.727 &0.390 &0.234 &0.383 &0.552\\
    \hline
     ~+\textbf{\emph{FourierMix}} &0.455 & 0.388 &0.326 &0.386 &0.453\\
      ~~+JSD &\underline{0.522} & \underline{0.444} &\underline{0.375} &\underline{0.454} &0.504 &0.295 & 0.247 &0.190 &0.258 &\underline{0.292} &\textbf{0.751} &\textbf{0.399} &\textbf{0.242} &\textbf{0.389} &0.564 &0.515\\
      
      ~~+\textbf{HCR} &\textbf{0.535} & \textbf{0.460} &\textbf{0.384} &\textbf{0.473} &\textbf{0.521} &\textbf{0.309} & \textbf{0.261} &\textbf{0.199} &\textbf{0.278} &\textbf{0.307} & \underline{0.750} &\underline{0.397} &\underline{0.239} &\underline{0.387} &\underline{0.567} \\
\noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
  \end{tabular}

==> sections/originaltables.tex <==
\begin{table*}[t]
\scriptsize
\renewcommand\arraystretch{0.9}
\setlength\tabcolsep{2.5pt}
  \caption{\small Models trained with \emph{FourierMix} and HCR achieve significant improvements in the certified robustness (ACR) guarantees on all corruption types from the CIFAR-10-C dataset.  %$\sigma=0.25$ is used for certification with RS and model training.
  %for Different Data Augmentations. 
  \textbf{Bold} and \underline{underline} denote the best and runner-up results, for all tables in this work. 
  %\BK{Better caption with message/results -- eg see winning hand captions}\AM{Move the detailed result to Appendix and only keep first 5 columns.}
  }
  \label{tb:cifar10c}
  \vspace{-0.2cm}
  \centering
  \begin{tabular}{|l|c|cccc|ccccccccccccccc|}
    \noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}

    %Pretext Task     & Parameters  &Clean Accuracy &Adv. Accuracy  &Clean Accuracy &Adv. Accuracy  &Clean Accuracy &Adv. Accuracy\\
    Augmentation    &clean & mACR &-low &-mid &-high  &Gauss. &Shot  &Impulse  &Defocus   &Glass  &Motion &Zoom &Snow  &Frost  &Fog  &Bright  &Contrast &Elastic &Pixel  &JPEG \\
\noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}     
    Gaussian &0.461 & 0.363 &0.301 &0.353 &0.435 &0.448 &0.448 &0.421 &0.380 &0.346 &0.338 &0.357 &0.394 &0.347 &0.187 &0.439 &0.137 &0.342 &0.420 &0.440\\
     ~+JSD &\textbf{0.535} & 0.439 &0.346 &0.451 &\underline{0.520} &\textbf{0.529} &\underline{0.514} &\textbf{0.528} &0.471 &0.445 &0.443 &0.453 &0.449 &0.378 &0.235 &0.485 &0.185 &0.444 &\underline{0.506} &\underline{0.521}\\
    \hline
     ~+AutoAugment &0.411  & 0.372 &0.312 &0.364 &0.431 &0.451 &0.452 &0.419 &0.411 &0.356 &0.342 &0.360 &0.403 &0.354 &0.201 &0.446 &0.158 &0.352 &0.429 &0.445\\
      ~~+JSD  &0.432 & 0.400 &0.343 &0.395 &0.464 &0.473 &0.476 &0.443 &0.423 &0.385 &0.394 &0.390 &0.427 &0.403 &0.212 &0.483 &0.189 &0.382 &0.453 &0.473\\
    \hline
     ~+AugMix &0.452 & 0.385 &0.324 &0.383 &0.449 &0.459 &0.460 &0.436 &0.412 &0.369 &0.372 &0.391 &0.413 &0.374 &0.216 &0.457 &0.159 &0.371 &0.439 &0.453\\
      ~~+JSD &0.518 & 0.430 &0.357 &0.436 &0.496 &0.504 &0.507 &0.481 &0.461 &0.426 &0.429 &0.441 &0.452 &0.408 &0.240 &0.501 &0.185 &0.425 &0.485 &0.502\\
      ~~+\textbf{HCR} &0.520 &0.437 &0.369 &0.444 &0.497 &0.505 &0.506 &0.484 &0.464 &0.438 &0.435 &0.447 &0.460 &0.426 &0.252 &0.505 &0.200 &0.437 &0.487 &0.501\\
    \hline
     ~+\textbf{\emph{FourierMix}} &0.455 & 0.388 &0.326 &0.386 &0.453 &0.461 &0.462 &0.446 &0.417 &0.369 &0.378 &0.393 &0.415 &0.376 &0.220 &0.457 &0.160 &0.373 &0.439 &0.456\\
      ~~+JSD &\underline{0.522} & \underline{0.444} &\underline{0.375} &\underline{0.454} &0.504 &0.512 &0.513 &0.491 &\underline{0.474} &\underline{0.448} &\underline{0.446} & \underline{0.456} &\underline{0.464} &\underline{0.432} &\underline{0.257} &\textbf{0.519} &\underline{0.201} &\underline{0.445} &0.495 &0.508\\
      
      ~~+\textbf{HCR} &\textbf{0.535} & \textbf{0.460} &\textbf{0.384} &\textbf{0.473} &\textbf{0.521} &\underline{0.528} &\textbf{0.530} &\underline{0.513} &\textbf{0.492} &\textbf{0.470} &\textbf{0.464} &\textbf{0.477} &\textbf{0.477} &\textbf{0.432} &\textbf{0.275} &\underline{0.517} &\textbf{0.220} &\textbf{0.462} &\textbf{0.511} &\textbf{0.524}\\
\noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
  \end{tabular}
  \vspace{-0.2cm}
\end{table*}


\begin{table*}[h]
\scriptsize
\renewcommand\arraystretch{0.9}
\setlength\tabcolsep{2.0pt}
  \caption{\small Improvement in the Average Certified Radius (ACR) of models trained with \emph{FourierMix} and HCR against CIFAR-100-C corruptions. 
  %$\sigma=0.25$ is used for certification with RS and model training. 
  \AM{Can be moved to Appendix due to space limitation}}
   \label{tb:cifar100c}
   \vspace{-0.2cm}
  \centering
  \begin{tabular}{|l|c|cccc|ccccccccccccccc|}
    \noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
    %Pretext Task     & Parameters  &Clean Accuracy &Adv. Accuracy  &Clean Accuracy &Adv. Accuracy  &Clean Accuracy &Adv. Accuracy\\
    Augmentation  & clean   & mACR &-low &-mid &-high &Gauss. &Shot  &Impulse  &Defocus   &Glass  &Motion &Zoom &Snow  &Frost  &Fog   &Bright  &Contrast &Elastic &Pixel  &JPEG \\
    \noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
    Gaussian & 0.238 & 0.169 &0.131 &0.182 &0.208 & 0.214 &0.218 &0.193 &0.181 &0.170 &0.157 &0.169 &0.177 &0.153 &0.069 &0.207 &0.051 &0.159 &0.206 &0.209\\
    ~+JSD & 0.291 & 0.232 &0.167 &0.248 &0.280 &0.283 &0.285 &0.273 &0.261 &0.252 &0.240 &0.250 &0.226 &0.188 &0.104 &0.242 &0.079 &0.235 &0.278 &0.281\\
    \hline
     ~+AutoAugment + JSD &0.265 & 0.225 &0.175 &0.234 &0.265 &0.275 &0.273 &0.252 &0.248 &0.230 &0.230 &0.238 &0.232 &0.202 &0.104 &0.257 &0.082 &0.225 &0.261 &0.266\\
    \hline
     ~+AugMix + JSD & 0.286 & 0.231 &0.184 &0.240 &0.269 &0.274 &0.278 &0.256 &0.255 &0.236 &0.233 &0.243 &0.239 &0.211 &0.111 &0.267 &0.092 &0.232 &0.267 &0.270\\
     ~+AugMix + \textbf{HCR} &\underline{0.296}  &\underline{0.249} &\underline{0.191} &\underline{0.263} &\underline{0.292} &\underline{0.296} &\underline{0.301} &0.282 &\underline{0.278} &\underline{0.264} &\underline{0.255} &\underline{0.263} &0.249 &0.215 &\underline{0.118} &0.274 &\underline{0.097} &\underline{0.253} &\underline{0.291} &\underline{0.292}\\
    \hline
     ~+\emph{FourierMix} + JSD &0.295 & 0.247 &0.190 &0.258 &\underline{0.292} &0.295 &0.300 &\underline{0.283} &0.273 &0.257 &0.249 &0.260 &\underline{0.251} &\underline{0.217} &0.115 &\underline{0.275} &0.092 &0.250 &0.288 &\underline{0.292}\\
     ~+\textbf{\emph{FourierMix} + HCR} &\textbf{0.309} & \textbf{0.261} &\textbf{0.199} &\textbf{0.278} &\textbf{0.307} &\textbf{0.310} &\textbf{0.313} &\textbf{0.302} &\textbf{0.291} &\textbf{0.283} &\textbf{0.270} &\textbf{0.277} &\textbf{0.260} &\textbf{0.221} &\textbf{0.128} &\textbf{0.284} &\textbf{0.102} &\textbf{0.267} &\textbf{0.303} &\textbf{0.307}\\
\noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
  \end{tabular}
\end{table*}



